Continuous-Time Model-Based Reinforcement Learning

Model-based reinforcement learning (MBRL) approaches rely on discrete-time state transition models whereas physical systems and the vast majority of control tasks operate in continuous-time. To avoid time-discretization approximation of the underlying process, we propose a continuous-time MBRL framework based on a novel actor-critic method. Our approach also infers the unknown state evolution differentials with Bayesian neural ordinary differential equations (ODE) to account for epistemic uncertainty. We implement and test our method on a new ODE-RL suite that explicitly solves continuous-time control systems. Our experiments illustrate that the model is robust against irregular and noisy data, is sample-efficient, and can solve control problems which pose challenges to discrete-time MBRL methods.

==> old/old_fig5.tex <==

\begin{figure*}[t]
    \centering
\begin{minipage}[h]{0.01\textwidth}
    \centering
    \vspace{1cm}
    \rotatebox[origin=c]{90}{\textsc{Observation Noise}}
\end{minipage}
\hfill
\begin{minipage}[h]{0.97\textwidth}
    \centering
    \textsc{Observation Spacing} \par\medskip
    \begin{minipage}[t]{0.02 \textwidth}
        \centering
        \vspace{0.35cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.0$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\Dt = 0.1$
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\Dt \sim \mathcal{U}(0,0.2)$
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.000-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\Dt \sim \text{Exp}(10)$
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.000-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.5cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.01$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.010-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.010-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.010-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.6cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.025$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.025-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.025-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp5/cartpole-0.100-0.025-exp.png}
    \end{minipage}
\end{minipage}
\caption{A comparison of ENODE and MPETS on CartPole environment. We illustrate how the mean reward and 90/10 quantiles over rounds behave across different observation spacings and noise levels. Note that all three spacings have the same mean time increments $\dt=0.1$. We observe that MPETS quickly deteriorates with irregular sampling and increased noise while our model is robust up to certain thresholds. We also see that combined effects are more harmful on both models.}
\label{fig:exp2}
\end{figure*}


==> old/old_fig6.tex <==
\begin{figure*}[!h]
    \centering
\begin{minipage}[h]{0.01\textwidth}
    \centering
    \vspace{1cm}
    \rotatebox[origin=c]{90}{\textsc{Mean Time Difference}}
\end{minipage}
\hfill
\begin{minipage}[h]{0.97\textwidth}
    \centering
    % \textsc{Observation Spacing} \par\medskip
    \begin{minipage}[t]{0.02 \textwidth}
        \centering
        \vspace{0.45cm}
        \rotatebox[origin=c]{90}{\scriptsize $\kappa=0.1$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\dt = \kappa$
        \includegraphics[width=\linewidth]{exp3/pendulum-0.100-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\dt \sim \mathcal{U}(0,2\kappa)$
        \includegraphics[width=\linewidth]{exp3/pendulum-0.100-0.000-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\dt \sim \text{Exp}(1/\kappa)$
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.000-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.5cm}
        \rotatebox[origin=c]{90}{\scriptsize $\kappa=0.2$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.200-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.200-0.000-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.200-0.000-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.6cm}
        \rotatebox[origin=c]{90}{\scriptsize $\kappa=0.4$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.400-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.400-0.000-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp3/pendulum-0.400-0.000-exp.png}
    \end{minipage}
\end{minipage}
\caption{A comparison of ENODE and MPETS on Pendulum environment with three different observation spacings and varying the mean time difference $\kappa$. Increased $\dt$ and irregular sampling influence MPETS negatively while our method is more robust to these changes.}
\label{fig:exp3}
\end{figure*}


==> old/sfig3.tex <==

\begin{figure*}[h]
    \centering
\begin{minipage}[h]{0.01\textwidth}
    \centering
    \vspace{1cm}
    \rotatebox[origin=c]{90}{\textsc{Observation Noise}}
\end{minipage}
\hfill
\begin{minipage}[h]{0.97\textwidth}
    \centering
    \textsc{Observation Spacing} \par\medskip
    \begin{minipage}[t]{0.02 \textwidth}
        \centering
        \vspace{0.35cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.0$}
    \end{minipage}
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        $\Dt = 0.1$
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        $\Dt \sim \mathcal{U}(0,0.2)$
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.000-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.31\textwidth}
        \centering
        $\Dt \sim \text{Exp}(10)$
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.000-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.5cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.01$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.010-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.010-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.010-exp.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.6cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.025$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.025-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.025-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.025-exp.png}
    \end{minipage}
    \vfill
    % \begin{minipage}[t]{0.02\textwidth}
    %     \centering
    %     \vspace*{-1.5cm}
    %     \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.05$}
    % \end{minipage}
    % \begin{minipage}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.050-fixed.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.050-uniform.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.32\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.050-exp.png}
    % \end{minipage}
    % \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.5cm}
        \rotatebox[origin=c]{90}{\scriptsize $\sigma=0.1$}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.100-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.100-uniform.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp2/pendulum-0.100-0.100-exp.png}
    \end{minipage}
\end{minipage}
\caption{We repeat the experiment in Section. 6.4 on the Pendulum environment. We again observe our model consistently outperforming MPETS while the performance slightly worsens with increased irregularity and noise.}
\label{fig:pend}
\end{figure*}


==> old/sfig4.tex <==

\begin{figure*}[h]
    \centering
\begin{minipage}[h]{0.01\textwidth}
    \centering
    \vspace{1cm}
    \rotatebox[origin=c]{90}{\textsc{Mean Time Difference}}
\end{minipage}
\hfill
\begin{minipage}[h]{0.97\textwidth}
    \centering
    \textsc{Observation Noise} \par\medskip
    \begin{minipage}[t]{0.02 \textwidth}
        \centering
        \vspace{0.45cm}
        \rotatebox[origin=c]{90}{\scriptsize $\Dt=0.1$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\sigma = 0.0$
        \includegraphics[width=\linewidth]{exp4/pendulum-0.100-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\sigma = 0.025$
        \includegraphics[width=\linewidth]{exp4/pendulum-0.100-0.025-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        $\sigma = 0.05$
        \includegraphics[width=\linewidth]{exp4/pendulum-0.100-0.050-fixed.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.5cm}
        \rotatebox[origin=c]{90}{\scriptsize $\Dt=0.2$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.200-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.200-0.025-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.200-0.050-fixed.png}
    \end{minipage}
    \vfill
    \begin{minipage}[t]{0.02\textwidth}
        \centering
        \vspace*{-1.6cm}
        \rotatebox[origin=c]{90}{\scriptsize $\Dt=0.4$} 
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.400-0.000-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.400-0.025-fixed.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{exp4/pendulum-0.400-0.050-fixed.png}
    \end{minipage}
\end{minipage}
\caption{We compare ENODE and PETS on three different observation spacings and also vary the fixed time difference $\Dt$ between observations. With increased $\Dt$ and irregular sampling, MPETS' performance significantly worsens while our method is more robust to changes.}
\label{fig:pend2}
\end{figure*}

